DEIM: DETR with Improved Matching for Fast Convergence

We introduce DEIM, an innovative and efficient training framework designed to accelerate convergence in real-time object detection with Transformer-based architectures (DETR). To mitigate the sparse supervision inherent in one-to-one (O2O) matching in DETR models, DEIM employs a Dense O2O matching strategy. This approach increases the number of positive samples per image by incorporating additional targets, using standard data augmentation techniques. While Dense O2O matching speeds up convergence, it also introduces numerous low-quality matches that could affect performance. To address this, we propose the Matchability-Aware Loss (MAL), a novel loss function that optimizes matches across various quality levels, enhancing the effectiveness of Dense O2O. Extensive experiments on the COCO dataset validate the efficacy of DEIM. When integrated with RT-DETR and D-FINE, it consistently boosts performance while reducing training time by 50%. Notably, paired with RT-DETRv2, DEIM achieves 53.2% AP in a single day of training on an NVIDIA 4090 GPU. Additionally, DEIM-trained real-time models outperform leading real-time object detectors, with DEIM-D-FINE-L and DEIM-D-FINE-X achieving 54.7% and 56.5% AP at 124 and 78 FPS on an NVIDIA T4 GPU, respectively, without the need for additional data. We believe DEIM sets a new baseline for advancements in real-time object detection. Our code and pre-trained models are available at https://github.com/ShihuaHuang95/DEIM.

==> sec/others.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Impact of Dense O2O and \ourclsloss.} We conduct experiments with ResNet50~\cite{he2016deep} and ResNet101~\cite{he2016deep}. Experiments are conducted on COCO~\cite{lin2014microsoft} and we report the performance on COCO~\cite{lin2014microsoft} val2017.}
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{lcccccc}
    \toprule
    Epochs & Dense O2O & \ourclsloss & AP & AP$_{50}$ & AP$_{75}$ \\
    \hline
    \rowcolor{f2ecde}
    \multicolumn{6}{c}{\textbf{ResNet50~\cite{he2016deep}-based}} \\
    72  &  &   & 53.4 & 71.6 & 57.4 \\
    \hline
    \multirow{2}{*}{36} % & \checkmark &  & 53.2 & 71.4 & 57.8 \\
                        % & \checkmark & \checkmark & 53.4 & 71.3 & 57.9 \\
                        & \checkmark &  & 53.6 & 71.2 & 57.8 \\   % ToBe Done
                        & \checkmark & \checkmark & 53.6 & 71.4 & 58.0 \\
    % \hline
    % \multirow{2}{*}{48} & \checkmark &  & 53.7 & 71.9 & 58.1 \\
    %                     & \checkmark & \checkmark & 53.8 & 71.8 & 58.3 \\
    \midrule
    \rowcolor{f2ecde}
    \multicolumn{6}{c}{\textbf{ResNet101~\cite{he2016deep}-based}} \\
    72  &  &  & 54.3 & 72.9 & 58.8 \\
    \hline
    \multirow{2}{*}{36} % & \checkmark &  & 54.1 & 72.3 & 58.4 \\
                        % & \checkmark & \checkmark & 54.5 & 72.5 & 59.2 \\
                        & \checkmark &  & 55.1 & 72.8 & 59.1 \\   % ToBe Done
                        & \checkmark & \checkmark & 55.2 & 73.3 & 59.9 \\
    % \hline
    % \multirow{2}{*}{48} & \checkmark &  & 54.5 & 72.9 & 58.9 \\
    %                     & \checkmark & \checkmark & 55.0 & 73.0 & 59.8 \\
    \midrule
\end{tabular}
}
\vspace{-0.4cm}
\label{tab:ab_all} 
\end{table}

Table~\ref{tab:ab_all} presents the effectiveness of the two core components: Dense O2O and \ourclsloss. Dense O2O significantly accelerates model convergence, achieving performance similar to the baseline after just 36 epochs, as opposed to the 72 epochs required for the original model. When combined with \ourclsloss, our method further improves performance, especially on the ResNet101~\cite{he2016deep} backbone, where we observe a 0.5 AP increase. This improvement is largely driven by better box quality, as evidenced by a 0.8 AP$_{75}$ gain, aligning with our goal of optimizing low-quality matches to improve high-quality box predictions. Overall, Dense O2O and \ourclsloss\ consistently deliver performance gains across both ResNet50~\cite{he2016deep} and ResNet101~\cite{he2016deep} backbones, demonstrating their robustness and generalizability.

\noindent \textbf{Effectiveness of Dense O2O and \ourclsloss{} on D-FINEs~\cite{peng2024d}.} We further validate the effectiveness of Dense O2O and our loss within the D-FINE framework, observing consistent improvements from both components (~\Cref{tab:ab_dfine_all}). Additionally, the improvement is most notable in AP$_{75}$, approaching a 1\% increase, indicating more accurate predictions.

\begin{table}[htbp]
\centering
\caption{\textbf{Impact of Dense O2O and \ourclsloss{} on D-FINEs.}}
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{lcccccc}
    \toprule
    Epoch & Dense O2O & \ourclsloss & AP & AP$_{50}$ & AP$_{75}$ \\
    \hline
    \rowcolor{f2ecde}
    \multicolumn{6}{c}{\textbf{D-FINE-L-based}} \\
    72 &  &   & 54.0 & 71.6 & 58.4 \\
    \hline
    \multirow{2}{*}{36} 
                        &  &  & 53.5 & 71.2 & 58.2 \\
                        & \checkmark &  & 54.2 & 72.1 & 58.9 \\
                        & \checkmark & \checkmark & 54.6 & 72.2 & 59.5 \\
    \midrule
    \rowcolor{f2ecde}
    \multicolumn{6}{c}{\textbf{D-FINE-X-based}} \\
    72 &  &  & 55.8 & 73.7 & 60.2 \\
    \hline
    \multirow{2}{*}{36} 
                        &  &  & 55.5 & 73.1 & 60.4 \\
                        & \checkmark &  & 56.0 & 73.6 & 60.9 \\
                        & \checkmark & \checkmark & 56.2 & 73.8 & 61.2 \\

    \midrule
\end{tabular}
}
\vspace{-0.7cm}
\label{tab:ab_dfine_all} 
\end{table}
